CodeTaxo: Enhancing Taxonomy Expansion with Limited Examples via Code Language Prompts

Taxonomies play a crucial role in various applications by providing a structural representation of knowledge. The task of taxonomy expansion involves integrating emerging concepts into existing taxonomies by identifying appropriate parent concepts for these new query concepts. Previous approaches typically relied on self-supervised methods that generate annotation data from existing taxonomies. However, these methods are less effective when the existing taxonomy is small (fewer than 100 entities). In this work, we introduce CodeTaxo, a novel approach that leverages large language models through code language prompts to capture the taxonomic structure. Extensive experiments on five real-world benchmarks from different domains demonstrate that CodeTaxo consistently achieves superior performance across all evaluation metrics, significantly outperforming previous state-of-the-art methods. The code and data are available at https://github.com/QingkaiZeng/CodeTaxo-Pub.

==> 1introduction-old.tex <==
Taxonomy has a hierarchical structure that represents the hypernym-hyponym relations or ``is-A'' relations between concepts or entities. Researchers have been using relational knowledge to identify semantic relevance for web search~\cite{yin2010building,liu2020giant, kang2024improving}, personalized recommendation~\cite{zhang2014taxonomy,tan2022enhancing,huang2019taxonomy}, and question answering~\cite{yang2017efficiently}. Existing taxonomies are mainly constructed by human experts or through crowd-sourcing, but this manual approach is time-consuming, labor-intensive, and often limited in knowledge coverage~\cite{bordea2016semeval,jurgens2016semeval}. As new entities continue to emerge, it becomes essential to keep these taxonomies up-to-date by enriching them with these emerging entities. To address the challenges of manual taxonomy construction and maintenance, taxonomy expansion tasks have been developed to automatically expand the existing taxonomies by integrating emerging entities into the relational graph~\cite{jurgens2016semeval}.

\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.45\textwidth}
   \includegraphics[width=\textwidth]{Figures/intro-part1.pdf}
   \caption{\textbf{Discriminative Methods:} A trained scoring function selects the most appropriate parent entity from the taxonomy for a given query entity.}
   \label{fig:motivation_sub1}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
   \includegraphics[width=\textwidth]{Figures/intro-part2.pdf}
   \caption{\textbf{Generative Methods:} LLMs generate the parent entity from the taxonomy based on the query entity.}
   \label{fig:motivation_sub2}
\end{subfigure}
\caption{Two Types Taxonomy Expansion Methods}
\vspace{-0.3in}
\label{fig:motivation}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{Figures/Framework-CodeTaxo.pdf}
    \vspace{-0.3in}
    \caption{The overview of the pipeline for \textsc{CodeTaxo}: \textsc{CodeTaxo} reformulates the task of integrating a query entity $q$ into an existing taxonomy $\mathcal{T}_0$ as a code completion task using code-based prompts for LLMs.}
    \label{fig:framework}
    \vspace{-0.2in}
\end{figure*}

As illustrated in Figure~\ref{fig:motivation_sub1}, recent approaches to taxonomy expansion primarily follow discriminative methods that model hierarchical structures derived from existing taxonomies using techniques like Egonets~\cite{shen2020taxoexpan}, mini-paths~\cite{yu2020steam}, and Ego-Trees~\cite{wang2021enquire}. While pre-trained language models (PLMs) improve these methods by encoding entities’ textual descriptions to enrich semantic representations~\cite{wang2021enquire,wang2022qen, liu2021temp,xu2022taxoprompt}, their reliance on self-supervised annotations from small taxonomies often limits their effectiveness. In contrast, generative large language models (LLMs) such as GPT-4~\cite{achiam2023gpt} and the Llama family~\cite{touvron2023llama, dubey2024llama} excel at understanding and generating structural knowledge~\cite{ye2022generative, bi2024codekgc, sun2024head,sun2024large}, and scaling them up enhances generalization, enabling superior few-shot or zero-shot performance even with limited training data. As illustrated in Figure~\ref{fig:motivation_sub2}, these generative models draw on extensive pre-training knowledge to effectively expand taxonomies despite sparse self-supervision.


However, two key challenges arise when employing LLMs for taxonomy expansion. First, unlike traditional NLP tasks such as question answering and machine translation, which naturally align with text-to-text generation, the taxonomic structure required here is often difficult to represent as natural language. In particular, generating the taxonomy as the specialized graph structures mentioned in\cite{madaan2022language} must be serialized into text, which involves ``flattening'' the taxonomy into a sequence of parent-child entity pairs. However, LLMs are primarily pre-trained on unstructured text, making these serialized structured outputs considerably different from the majority of their pre-training data. Moreover, semantically related words are usually located within a relatively small range in natural language. In contrast, when representing a taxonomy as a linear sequence, conceptually related entities may be positioned at greater distances from each other. Second, unlike the reasoning graph proposed in \cite{madaan2022language}, only limited amounts of state information can be used as input context. In large-scale taxonomy expansion, including the entire existing taxonomy in the prompt is infeasible due to current LLMs’ constrained context windows and associated computational costs. Even if it were possible to include thousands of entities, this would cause a loss of structural information, diminishing the LLM’s ability to discern entity-specific details.


To address these two challenges, we proposed \textsc{CodeTaxo}, a novel approach to taxonomy expansion that leverages code languages as prompts. Recent progress in large language models of code (Code-LLMs)~\cite{roziere2023code} has demonstrated the potential to employ Code-LLMs for different structure prediction tasks~\cite{madaan2022language, li2023codeie, wang2023code4struct,li2024knowcoder,bi2024codekgc}. The core philosophy of these approaches is that code language can more effectively represent structural data compared to natural language.  In \textsc{CodeTaxo}, we reformulate the taxonomy expansion task as a code completion problem to exploit the benefits of code languages. We first define a base class \texttt{Entity}, which encapsulates the surface name and definition of entities to represent their semantic information. Additionally, \texttt{Entity} class includes references to the parent entity and a list of child entities, thereby capturing the taxonomic relations among the entities. Two methods for modifying the taxonomic relations between entities are also included in the \texttt{Entity} class. To represent the existing taxonomy that we aim to expand, we instantiate the \texttt{Entity} class for each entity within the current taxonomy. To address the limitation posed by the contextual window size of LLMs, which cannot accommodate the entire taxonomy, we selectively include only entities that exhibit high similarity to the query entity in the prompt. For encoding the textual descriptions of entities, we utilize SimCSE~\cite{gao2021simcse}, measuring similarity through cosine similarity.


The effectiveness of \textsc{CodeTaxo} has been validated through extensive experiments on two sets of small-scale sub-taxonomies from WordNet~\cite{bansal2014structured}, Graphine~\cite{liu2021graphine}, and three large-scale taxonomies from SemEval-2016~\cite{bordea2016semeval}. The experimental result demonstrates that \textsc{CodeTaxo} in the one-shot setting outperforms all self-supervised baseline methods, despite these baselines being well-trained on self-supervised annotation data derived from large-scale taxonomies in SemEval-2016. Specifically, our \textsc{CodeTaxo} in the one-shot setting shows relative improvements in accuracy of 10.26\%, 8.89\%, and 9.21\% on SemEval-Sci, SemEval-Env, and SemEval-Food, respectively. Additionally, we evaluated \textsc{CodeTaxo} using various open-source LLMs, revealing several interesting observations discussed in this work.

In summary, our main contributions include:\begin{compactitem}
    \item We introduce \textsc{CodeTaxo}, an innovative in-context learning method that utilizes code language prompts to represent taxonomic relationships between entities, thereby improving the effectiveness of taxonomy expansion.
    \item We develop a similarity-based filter, which employs a small pre-trained model to encode the textual descriptions of entities, ensuring that only highly relevant entities are included in the prompt concerning the query entity.
    \item Extensive experiments demonstrate that \textsc{CodeTaxo} significantly enhances the performance of taxonomy expansion across two sets of small-scale sub-taxonomies and three large-scale taxonomies.
\end{compactitem}




% \indent \textbf{Scope and Limitation.} This study represents an initial effort to utilize LLMs for taxonomy expansion. Our primary objective is to identify an effective in-context learning strategy to leverage the potential of LLMs. We acknowledge that the performance and scalability of \textsc{CodeTaxo} are constrained by the inherent knowledge of LLMs and the limitations of their context window size. While this paper does not address the challenges of expanding LLM knowledge or increasing context window size, we hope that our work will inspire further research in these areas.



% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.0\linewidth]{Figures/Framework-CodeTaxo.pdf}
%     \vspace{-0.3in}
%     \caption{The overview of the pipeline for \textsc{CodeTaxo}: \textsc{CodeTaxo} reformulates the task of integrating a query entity $q$ into an existing taxonomy $\mathcal{T}_0$ as a code completion task using code-based prompts for LLMs.}
%     \label{fig:framework}
%     \vspace{-0.15in}
% \end{figure*}

